ZhiFangDanTai: Fine-tuning Graph-based Retrieval-Augmented Generation Model for Traditional Chinese Medicine Formula

Traditional Chinese Medicine (TCM) formulas play a significant role in treating epidemics and complex diseases. Existing models for TCM utilize traditional algorithms or deep learning techniques to analyze formula relationships, yet lack comprehensive results, such as complete formula compositions and detailed explanations. Although recent efforts have used TCM instruction datasets to fine-tune Large Language Models (LLMs) for explainable formula generation, existing datasets lack sufficient details, such as the roles of the formula's sovereign, minister, assistant, courier; efficacy; contraindications; tongue and pulse diagnosis-limiting the depth of model outputs. To address these challenges, we propose ZhiFangDanTai, a framework combining Graph-based Retrieval-Augmented Generation (GraphRAG) with LLM fine-tuning. ZhiFangDanTai uses GraphRAG to retrieve and synthesize structured TCM knowledge into concise summaries, while also constructing an enhanced instruction dataset to improve LLMs' ability to integrate retrieved information. Furthermore, we provide novel theoretical proofs demonstrating that integrating GraphRAG with fine-tuning techniques can reduce generalization error and hallucination rates in the TCM formula task. Experimental results on both collected and clinical datasets demonstrate that ZhiFangDanTai achieves significant improvements over state-of-the-art models. Our model is open-sourced at https://huggingface.co/tczzx6/ZhiFangDanTai1.0.

==> ref-1.tex <==
\begin{thebibliography}{00}\leftskip1pc
	\bibitem{1}Jing Tang.Research on mining method and application of TCM compatibility rule based on statistical learning theory[D].Nanjing University of Chinese Medicine,2024.DOI:10.27253/d.cnki.gnjzu.2024.000256.
	\bibitem{2}  	Ji Xiang Liu. Research on compatibility of traditional Chinese medicine based on big data thinking[D].,2017.
	\bibitem{3}  	Ni Ma et al. Application of complex network method in data mining of traditional Chinese medicine compound[J].2021, DOI: :1007-9416(2021)12-0068-03.
	\bibitem{4}  	Dong, X., Zhao, C., Song, X., et al. PresRecST: a novel herbal prescription recommendation algorithm for real-world patients with integration of syndrome differentiation and treatment planning. Journal of the American Medical Informatics Association, 31(6), 1268-1279, 2024.
	\bibitem{5}  	Jin Y, Ji W, Zhang W, He X, et al. A KG-enhanced multi-graph neural network for attentive herb recommendation, IEEE/ACM Transactions on Computational Biology and Bioinformatics, 2021.
	\bibitem{6}  	Li S, Wang W, He J, KGAPG: Knowledge-aware neural group representation learning for attentive prescription generation of traditional Chinese medicine, in 2021 IEEE International Conference on Bioinformatics and Biomedicine (BIBM). IEEE, 2021;450–455.
	\bibitem{7}  	Li W, Yang Z, Exploration on generating traditional chinese medicine  prescriptions from symptoms with an end-to-end approach, in CCF International Conference on Natural Language Processing and Chinese Computing. Springer, 2019; 486–498.
	\bibitem{8}  	Hu Y, Wen G, Liao H, et al. Automatic construction of chinese herbal prescriptions from tongue images using cnns and auxiliary latent therapy topics. IEEE Trans Cybernet. 2019;51(2):708–21.
	\bibitem{9}  	Liao H, Wen G, Hu Y, et al. Convolutional herbal prescription building method from multi-scale facial features, Multimedia Tools and Applications, vol. 78, no. 24, pp. 35 665–35 688, 2019.
	\bibitem{10}  	Zhou W, Yang K, Zeng J, et al. FordNet: recommending traditional Chinese medicine formula via deep neural network integrating phenotype and molecule. Pharmacol Res. 2021;173: 105752.
	\bibitem{11}  	Dong X, Zheng Y, Shu Z, et al., TCMPR: TCM prescription recommendation based on subnetwork term mapping and deep learning, in 2021 IEEE International Conference on Bioinformatics and Biomedicine (BIBM). IEEE, 2021;3776–3783.
	\bibitem{12}  	Dong X, Zhao C, Song X, et al. PresRecST: a novel herbal prescription recommendation algorithm for real-world patients with integration of syndrome diferentiation and treatment planning. J Am Med Inform Assoc. 2024;31(6):1268–79.
	\bibitem{13}  	Wang Z, Liang Y, Liu Z. FFBDNet: Feature fusion and bipartite decision networks for recommending medication combination, in Joint European Conference on Machine Learning and Knowledge Discovery in Databases.Springer, 2022;419–436.
	\bibitem{14}  	Tan W, Wang W, Zhou X, et al. OntoMedRec: Logically-pretrained model-agnostic ontology encoders for medication recommendation. World Wide Web. 2024;27(3):28.
	\bibitem{15}  	Mi J, Zu Y, Wang Z, et al. ACDNet: Attention-guided Collaborative Decision Network for efective medication recommendation. J Biomed Inform. 2024;149: 104570.
	\bibitem{16}  	Zheng Z, Wang C, Xu T, et al. Interaction-aware drug package recommendation via policy gradient. ACM Trans Inf Syst. 2023;41(1):1–32.
	\bibitem{17}  	Zhao, W., Lu, W., Li, Z., et al. TCM herbal prescription recommendation model based on multi-graph convolutional network. Journal of Ethnopharmacology, 297, 115109.
	\bibitem{18}  	Yang, K., Yu, Z., Su, X., et al. PrescDRL: deep reinforcement learning for herbal prescription planning in treatment of chronic diseases. Chinese Medicine, 19(1), 144.
	\bibitem{19}  	Z. Liu, Z. Zheng, X. Guo, L., et al, “Attentiveherb: a novel method for traditional medicine prescription generation,” IEEE Access, vol. 7, pp. 139 069–139 085, 2019.
	\bibitem{20}  	C. Li, D. Liu, K. Yang, X., et al. “Herb-know: Knowledge enhanced prescription generation for traditional chinese medicine,” in BIBM, 2020, pp. 1560–1567.
	\bibitem{21}  	Z. Liu, C. Luo, D. Fu, J., et al. “A novel transfer learning model for traditional herbal medicine prescription generation from unstructured resources and knowledge,” Artif. Intell. Med., vol. 124, p. 102232, 2022.
	\bibitem{22}  	H. Pu, J. Mi, S. Lu, et al. “Rokepg: Roberta and knowledge enhancement for prescription generation of traditional chinese medicine,” in BIBM, 2023, pp. 4615–4622.
	\bibitem{23}  	Dubey, A., Jauhri, A., Pandey, A., et al. The llama 3 herd of models. arXiv preprint arXiv:2407.21783, 2024.
	\bibitem{24}  	ZhipuAI, ChatGLM, 2024
	\bibitem{25}  	Zhou, X., Dong, X., Li, C.,  et al. TCM-FTP: Fine-Tuning Large Language Models for Herbal Prescription Prediction. arXiv preprint arXiv:2407.10510.
	\bibitem{26}  	Edge, D., Trinh, H., Cheng, N., et al. From local to global: A graph rag approach to query-focused summarization. arXiv preprint arXiv:2404.16130.
	\bibitem{27}  	Kimi, 2023, MoonShot.
	\bibitem{28}  	DeepSeek-v3, 2024.
	\bibitem{29}  	Robertson, S. Understanding inverse document frequency: on theoretical arguments for IDF. Journal of documentation, 60(5), 503-520.
	\bibitem{30}  	Bo, H., Yi, Lfei, Li, L., et al.The Instruction Tuning of Large Language Models with Multi-Modal Recommendation Instruction. Journal of Beijing University of Posts and Telecommunications, 2024, 47(4): 36-43.
	\bibitem{31}  	Lewis, P., Perez, E., Piktus, A., et al. Retrieval-augmented generation for knowledge-intensive nlp tasks. Advances in Neural Information Processing Systems, 33, 9459-9474, 2020.
	\bibitem{32}  	Zhou, C., Liu, P., Xu, P., et al. Lima: Less is more for alignment. Advances in Neural Information Processing Systems, 36, 2024.
	\bibitem{33}  	Rafailov, R., Sharma, A., Mitchell, E. Direct preference optimization: Your language model is secretly a reward model. Advances in Neural Information Processing Systems, 36, 2024.
	\bibitem{34}  	Zhang, T., Patil, S. G., Jain, N., et al. Raft: Adapting language model to domain specific rag. arXiv preprint arXiv:2403.10131, 2024.
	\bibitem{35}  	Dong, X., Zheng, Y., Shu, Z., et al. TCMPR: TCM prescription recommendation based on subnetwork term mapping and deep learning. BioMed Research International, 2022(1), 4845726.
	\bibitem{36}  	Yao, L., Zhang, Y., Wei, B., et al. A topic modeling approach for traditional Chinese medicine prescriptions. IEEE Transactions on Knowledge and Data Engineering, 30(6), 1007-1021, 2018.
	\bibitem{37}  	Xue, Z., Yang, K., Hao, T., et al. TCMLLM, https://github.com/2020MEAI/TCMLLM
	\bibitem{38}  	Lewis, P., Perez, E., Piktus, A., et al. Retrieval-augmented generation for knowledge-intensive nlp tasks. Advances in Neural Information Processing Systems, 33, 9459-9474, 2020.
	\bibitem{39}  	Dubey, A., Jauhri, A., Pandey, A., 2024. The Llama 3 Herd of Models. arXiv preprint arXiv:2407.21783.
	\bibitem{40}  	Ram, O., Levine, Y., Dalmedigos, I. et al. In-context retrieval-augmented language models. Transactions of the Association for Computational Linguistics, 11, 1316-1331, 2023.
	\bibitem{41}  	Ma, X., Gong, Y., He, P., et al. Query Rewriting in Retrieval-Augmented Large Language Models. In Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing (pp. 5303-5315), 2023.
	\bibitem{42}  	Anokhin, P., Semenov, N., Sorokin, A., et al. Arigraph: Learning knowledge graph world models with episodic memory for llm agents. arXiv preprint arXiv:2407.04363, 2024.
	\bibitem{43}  	Sarmah, B., Mehta, D., Hall, B., et al. Hybridrag: Integrating knowledge graphs and vector retrieval augmented generation for efficient information extraction. In Proceedings of the 5th ACM International Conference on AI in Finance (pp. 608-616), 2024
	\bibitem{44} 	Xiong, H., Bian, J., Li, Y., et al. When search engine services meet large language models: visions and challenges. IEEE Transactions on Services Computing, 2024.
	\bibitem{45}  	Hu, Y., Li, Z., Zhang, Z., et al. Hireview: Hierarchical taxonomy-driven automatic literature review generation. arXiv preprint arXiv:2410.03761, 2024
	\bibitem{46}  	Yan, S. Q., Gu, J. C., Zhu, Y. et al. Corrective retrieval augmented generation. arXiv preprint arXiv:2401.15884, 2024.
	\bibitem{47}  	Meister, C., Vieira, T., \& Cotterell, R. (2020). Best-first beam search. Transactions of the Association for Computational Linguistics, 8, 795-809.
	\bibitem{48}  	Qwen2.5, ByterDance, 2024.
	\bibitem{49} Jie, W. A. N. G., et al. "Research on multimodal social media information popularity prediction based on large language model." Journal on Communication/Tongxin Xuebao 45.11 (2024).
	\bibitem{50} Ouyang, L., Wu, J., Jiang, X., Almeida, D., Wainwright, C., Mishkin, P., ... \& Lowe, R. (2022). Training language models to follow instructions with human feedback. Advances in neural information processing systems, 35, 27730-27744.
	\bibitem{51} Traag, V. A., Waltman, L., and Van Eck, N. J. (2019). From Louvain to Leiden: guaranteeing well-connected communities. Scientific Reports, 9(1).
	\bibitem{52} Dean, J., \& Ghemawat, S. (2008). MapReduce: simplified data processing on large clusters. Communications of the ACM, 51(1), 107-113.
	
	
	

\end{thebibliography}

==> ref.tex <==
\begin{thebibliography}{00}\leftskip1pc
	\bibitem{1}Jing Tang.Research on mining method and application of TCM compatibility rule based on statistical learning theory[D].Nanjing University of Chinese Medicine,2024.DOI:10.27253/d.cnki.gnjzu.2024.000256.
	\bibitem{2}  	Ji Xiang Liu. Research on compatibility of traditional Chinese medicine based on big data thinking[D].,2017.
	\bibitem{3}  	Ni Ma et al. Application of complex network method in data mining of traditional Chinese medicine compound[J].2021, DOI: :1007-9416(2021)12-0068-03.
	\bibitem{4}  	Dong, X., Zhao, C., Song, X., et al.  “PresRecST: a novel herbal prescription recommendation algorithm for real-world patients with integration of syndrome differentiation and treatment planning,” J. Am. Med. Inform. Assoc., vol. 31, no. 6, pp. 1268–1279, 2024, doi: 10.1093/jamia/ocae066.  
	\bibitem{5}  	Jin, Y., Ji, W., Zhang, W., et al. “A KG-Enhanced Multi-Graph Neural Network for Attentive Herb Recommendation,” IEEE/ACM Trans. Comput. Biol. Bioinform., vol. 19, no. 5, pp. 2560–2571, 2022, doi: 10.1109/TCBB.2021.3115489.
	\bibitem{6}  	Li S, Wang W, He J, “KGAPG: Knowledge-Aware Neural Group Representation Learning for Attentive Prescription Generation of Traditional Chinese Medicine,” in Proceedings of the IEEE International Conference on Bioinformatics and Biomedicine (BIBM), 2021, pp. 450–455, doi: 10.1109/BIBM52615.2021.9669769. 
	\bibitem{7}  	Li W, Yang Z, “Exploration on generating traditional Chinese medicine prescriptions from symptoms with an end-to-end approach,” in Proceedings of the CCF International Conference on Natural Language Processing and Chinese Computing, 2019, pp. 486–498.
	\bibitem{8}  	Hu Y, Wen G, Liao H, et al., “Automatic construction of Chinese herbal prescriptions from tongue images using CNNs and auxiliary latent therapy topics,” IEEE Trans. Cybern., vol. 51, no. 2, pp. 708–721, 2019, doi: 10.1109/TCYB.2019.2909925. 
	\bibitem{9}  	Liao H, Wen G, Hu Y, et al., “Convolutional herbal prescription building method from multi-scale facial features,” Multimedia Tools Appl., vol. 78, no. 24, pp. 35665–35688, 2019, doi: 10.1007/s11042-019-08118-7.
	\bibitem{10}  	Zhou W, Yang K, Zeng J, et al., “FordNet: recommending traditional Chinese medicine formula via deep neural network integrating phenotype and molecule,” Pharmacol. Res., vol. 173, p. 105752, 2021, doi: 10.1016/j.phrs.2021.105752.
	\bibitem{11}  	Dong X, Zheng Y, Shu Z, et al., “TCMPR: TCM prescription recommendation based on subnetwork term mapping and deep learning,” in Proceedings of the IEEE International Conference on Bioinformatics and Biomedicine (BIBM), 2021, pp. 3776–3783, doi: 10.1109/BIBM52615.2021.9669768.
	\bibitem{12}  	Dong X, Zhao C, Song X, et al., “PresRecST: a novel herbal prescription recommendation algorithm for real-world patients with integration of syndrome differentiation and treatment planning,” J. Am. Med. Inform. Assoc., vol. 31, no. 6, pp. 1268–1279, 2024, doi: 10.1093/jamia/ocad066.
	\bibitem{13}  	Wang Z, Liang Y, Liu Z. “FFBDNet: Feature fusion and bipartite decision networks for recommending medication combination,” in Proceedings of the Joint European Conference on Machine Learning and Knowledge Discovery in Databases, 2022, pp. 419–436, doi: 10.1007/978-3-030-86523-8_28.
	\bibitem{14}  	Tan W, Wang W, Zhou X, et al., “OntoMedRec: Logically-pretrained model-agnostic ontology encoders for medication recommendation,” World Wide Web, vol. 27, no. 3, p. 28, 2024, doi: 10.1007/s11280-023-01112-7.
	\bibitem{15}  	Mi J, Zu Y, Wang Z, et al., “ACDNet: Attention-guided collaborative decision network for effective medication recommendation,” J. Biomed. Inform., vol. 149, p. 104570, 2024, doi: 10.1016/j.jbi.2023.104570.
	\bibitem{16}  	Zheng Z, Wang C, Xu T, et al., “Interaction-aware drug package recommendation via policy gradient,” ACM Trans. Inf. Syst., vol. 41, no. 1, pp. 1–32, 2023, doi: 10.1145/3548910.
	\bibitem{17}  	Zhao, W., Lu, W., Li, Z., et al., “TCM herbal prescription recommendation model based on multi-graph convolutional network,” J. Ethnopharmacol., vol. 297, p. 115109, 2022, doi: 10.1016/j.jep.2022.115109.
	\bibitem{18}  	Yang, K., Yu, Z., Su, X., et al., “PrescDRL: Deep reinforcement learning for herbal prescription planning in treatment of chronic diseases,” Chin. Med., vol. 19, no. 1, p. 144, 2024, doi: 10.1186/s13020-024-00822-9.
	\bibitem{19}  	Z. Liu, Z. Zheng, X. Guo, L., et al., “Attentiveherb: a novel method for traditional medicine prescription generation,” IEEE Access, vol. 7, pp. 139 069–139 085, 2019.
	\bibitem{20}  	C. Li, D. Liu, K. Yang, X., et al., “Herb-Know: Knowledge enhanced prescription generation for traditional Chinese medicine,” in Proceedings of the IEEE International Conference on Bioinformatics and Biomedicine (BIBM), 2020, pp. 1560–1567, doi: 10.1109/BIBM49941.2020.9313324.
	\bibitem{21}  	Z. Liu, C. Luo, D. Fu, J., et al., “A novel transfer learning model for traditional herbal medicine prescription generation from unstructured resources and knowledge,” Artif. Intell. Med., vol. 124, p. 102232, 2022, doi: 10.1016/j.artmed.2022.102232.
	\bibitem{22}  	H. Pu, J. Mi, S. Lu, et al., “ROKEPG: RoBERTa and knowledge enhancement for prescription generation of traditional Chinese medicine,” in Proceedings of the IEEE International Conference on Bioinformatics and Biomedicine (BIBM), 2023, pp. 4615–4622, doi: 10.1109/BIBM57880.2023.10326532.
	\bibitem{23}  	Dubey, A., Jauhri, A., Pandey, A., et al., “The LLaMA 3 herd of models,” arXiv preprint, arXiv:2407.21783, 2024.
	\bibitem{24}  	ZhipuAI, ChatGLM, 2024
	\bibitem{25}  	Zhou, X., Dong, X., Li, C.,  et al., “TCM-FTP: Fine-tuning large language models for herbal prescription prediction,” arXiv preprint, arXiv:2407.10510, 2024.
	\bibitem{26}  	Edge, D., Trinh, H., Cheng, N., et al., “From local to global: A graph RAG approach to query-focused summarization,” arXiv preprint, arXiv:2404.16130, 2024.
	\bibitem{27}  	Kimi, 2023, MoonShot.
	\bibitem{28}  	DeepSeek-v3, 2024.
	\bibitem{29}  	Robertson, S. “Understanding inverse document frequency: On theoretical arguments for IDF,” J. Doc., vol. 60, no. 5, pp. 503–520, 2004, doi: 10.1108/00220410410560582.
	\bibitem{30}  	Bo, H., Yi, Lfei, Li, L., et al., “The instruction tuning of large language models with multi-modal recommendation instruction,” J. Beijing Univ. Posts Telecommun., vol. 47, no. 4, pp. 36–43, 2024, doi: 10.19729/j.cnki.1004-0258.2024.04.004.
	\bibitem{31}  	Lewis, P., Perez, E., Piktus, A., et al., “Retrieval-augmented generation for knowledge-intensive NLP tasks,” Adv. Neural Inf. Process. Syst., vol. 33, pp. 9459–9474, 2020.
	\bibitem{32}  	Zhou, C., Liu, P., Xu, P., et al., “LIMA: Less is more for alignment,” Adv. Neural Inf. Process. Syst., vol. 36, 2024.
	\bibitem{33}  	Rafailov, R., Sharma, A., Mitchell, E. “Direct preference optimization: Your language model is secretly a reward model,” Adv. Neural Inf. Process. Syst., vol. 36, 2024.
	\bibitem{34}  	Zhang, T., Patil, S. G., Jain, N., et al., “RAFT: Adapting language model to domain specific RAG,” arXiv preprint, arXiv:2403.10131, 2024.
	\bibitem{35}  	Dong, X., Zheng, Y., Shu, Z., et al., “TCMPR: TCM prescription recommendation based on subnetwork term mapping and deep learning,” BioMed Res. Int., vol. 2022, no. 1, p. 4845726, 2022, doi: 10.1155/2022/4845726.
	\bibitem{36}  	Yao, L., Zhang, Y., Wei, B., et al., “A topic modeling approach for traditional Chinese medicine prescriptions,” IEEE Trans. Knowl. Data Eng., vol. 30, no. 6, pp. 1007–1021, 2018, doi: 10.1109/TKDE.2017.2784438.
	\bibitem{37}  	Xue, Z., Yang, K., Hao, T., et al. TCMLLM, https://github.com/2020MEAI/TCMLLM
	\bibitem{38}  	Lewis, P., Perez, E., Piktus, A., et al., “Retrieval-augmented generation for knowledge-intensive NLP tasks,” Adv. Neural Inf. Process. Syst., vol. 33, pp. 9459–9474, 2020.
	\bibitem{39}  	A. Dubey, A. Jauhri, A. Pandey, “The LLaMA 3 herd of models,” arXiv preprint, arXiv:2407.21783, 2024.
	\bibitem{40}  	Ram, O., Levine, Y., Dalmedigos, I. et al., “In-context retrieval-augmented language models,” Trans. Assoc. Comput. Linguist., vol. 11, pp. 1316–1331, 2023, doi: 10.1162/tacl_a_00567.
	\bibitem{41}  	Ma, X., Gong, Y., He, P., et al., “Query rewriting in retrieval-augmented large language models,” in Proc. Conf. Empirical Methods in Natural Language Process. (EMNLP), pp. 5303–5315, 2023.
	\bibitem{42}  	Anokhin, P., Semenov, N., Sorokin, A., et al., “ARIGraph: Learning knowledge graph world models with episodic memory for LLM agents,” arXiv preprint, arXiv:2407.04363, 2024.
	\bibitem{43}  	Sarmah, B., Mehta, D., Hall, B., et al., “HybridRAG: Integrating knowledge graphs and vector retrieval augmented generation for efficient information extraction,” in Proc. 5th ACM Int. Conf. AI Finance, pp. 608–616, 2024.
	\bibitem{44} 	Xiong, H., Bian, J., Li, Y., et al., “When search engine services meet large language models: Visions and challenges,” IEEE Trans. Serv. Comput., 2024, doi: 10.1109/TSC.2024.3276912.
	\bibitem{45}  	Hu, Y., Li, Z., Zhang, Z., et al., “HiReview: Hierarchical taxonomy-driven automatic literature review generation,” arXiv preprint, arXiv:2410.03761, 2024.
	\bibitem{46}  	Yan, S. Q., Gu, J. C., Zhu, Y. et al., “Corrective retrieval-augmented generation,” arXiv preprint, arXiv:2401.15884, 2024.
	\bibitem{47}  	C. Meister, T. Vieira, R. Cotterell, “Best-first beam search,” Trans. Assoc. Comput. Linguist., vol. 8, pp. 795–809, 2020, doi: 10.1162/tacl_a_00353.
	\bibitem{48}  	Qwen2.5, ByterDance, 2024.
	\bibitem{49} 	Jie, W. A. N. G., et al., “Research on multimodal social media information popularity prediction based on large language model,” J. Commun. (Tongxin Xuebao), vol. 45, no. 11, 2024.
	\bibitem{50} 	L. Ouyang, J. Wu, X. Jiang, et al., “Training language models to follow instructions with human feedback,” Adv. Neural Inf. Process. Syst., vol. 35, pp. 27730–27744, 2022.
	\bibitem{51} 	Traag, V. A., Waltman, L., and Van Eck, N. J. (2019). “From Louvain to Leiden: Guaranteeing well-connected communities,” Sci. Rep., vol. 9, no. 1, 2019, doi: 10.1038/s41598-019-41695-z.
	\bibitem{52} 	Dean, J., \& Ghemawat, S. (2008). “MapReduce: Simplified data processing on large clusters,” Commun. ACM, vol. 51, no. 1, pp. 107–113, 2008, doi: 10.1145/1327452.1327492.
	
	
	

\end{thebibliography}
